LLM-Blender: Ensembling Large Language Models with Pairwise Ranking and Generative Fusion

We present LLM-Blender, an ensembling framework designed to attain consistently superior performance by leveraging the diverse strengths of multiple open-source large language models (LLMs). Our framework consists of two modules: PairRanker and GenFuser, addressing the observation that optimal LLMs for different examples can significantly vary. PairRanker employs a specialized pairwise comparison method to distinguish subtle differences between candidate outputs. It jointly encodes the input text and a pair of candidates, using cross-attention encoders to determine the superior one. Our results demonstrate that PairRanker exhibits the highest correlation with ChatGPT-based ranking. Then, GenFuser aims to merge the top-ranked candidates, generating an improved output by capitalizing on their strengths and mitigating their weaknesses. To facilitate large-scale evaluation, we introduce a benchmark dataset, MixInstruct, which is a mixture of multiple instruction datasets featuring oracle pairwise comparisons. Our LLM-Blender significantly outperform individual LLMs and baseline methods across various metrics, establishing a substantial performance gap.

==> sections/1_introduction_old.tex <==


\section{Introduction}
\label{sec:intro}
 
% The fundamental goal of natural language generation is to generate coherent, reasonable, and task-specific texts with human-designed models. Nowadays, inspired by masked language pre-training objective from BERT\cite{devlin2018bert}, pre-training sequence-to-sequence models, like T5\cite{t5}, BART\cite{lewis2019bart}, PEGASUS\cite{zhang2020pegasus}, have surpassed i


% \todo{NLG in general; 
% Pre-trained seq2seq LMs (such as BART).
% Focus: decoding methods -- 4 different methods; 
% Findings: the gap between oracle selection VS top-beam performance.
% Motivation: closing this gap with reranking methods. mention some results refer to our Sec 4.4 } 

% Pre-trained encoder-decoder language models (LMs) have been proven effective for a wide range of natural language generation (NLG) tasks. 
% For example, BART \cite{lewis2019bart} adopts a denoising autoencoder architecture, training the model to recover the original sentence corrupted in various ways. T5 \cite{t5} conducted a systematic exploration of better pre-training methods. Other task-specific pre-trained models, such as PEGASUS \cite{zhang2020pegasus} for summarization tasks, have also shown great performance.



% To exploit these encoder-decoder LMs for NLG tasks,
% it is very important to use a suitable decoding method.
% Decoding methods such as beam search~\cite{}, diverse beam search~\cite{Vijayakumar2016DiverseBS}, top-k sampling~\cite{}, and top-p sampling~\cite{Holtzman2019TheCC} have been widely adopted during inference time.
% \todo{add citations}
% They are either greedy algorithms or sampling-based methods, and thus the final generation results of these methods are often not the best choices. 
% Prior studies \cite{cohen2019empirical,meister2020if, Ravaut2022SummaRerankerAM} found that top-beam results are usually much worse than the oracle selections from overly generated candidates.
% Also, if one could select the best output from the results of multiple decoding methods, then such oracle performance can be hugely improved.


% Pre-trained encoder-decoder language models (LMs) have demonstrated their effectiveness in various natural language generation (NLG) tasks. BART \cite{lewis2019bart} employs a denoising autoencoder architecture, in which the model is trained to reconstruct the original sentence from corruptions introduced during the training process. T5 \cite{t5} conducted a comprehensive study of alternative pre-training methods. Additionally, task-specific pre-trained models, such as PEGASUS \cite{zhang2020pegasus} for summarization tasks, have demonstrated impressive performance.


In order to effectively use language models (LMs) for natural language generation (NLG) tasks, it is crucial to employ an appropriate decoding method. Various decoding approaches, including beam search, diverse beam search~\cite{Vijayakumar2016DiverseBS}, top-k sampling, and top-p sampling~\cite{Holtzman2019TheCC}, have been widely employed to use LMs. 
These decoding methods, however, often produce suboptimal results. 
Previous studies \cite{cohen2019empirical,meister2020if, Ravaut2022SummaRerankerAM} have found that the top-beam generation results are frequently inferior to the oracle selections from the candidates generated by these methods. 
The oracle performance can be significantly improved by selecting the best output from the results of multiple decoding methods.


% We show an empirical analysis in Table~\ref{tab:main_oracle_gap}, where we look at three typical NLG tasks: summarization (CNN/DM), machine translation (WMT18), and constrained text generation (CommonGen). 
% For example, using the PEAGUS~\cite{zhang2020pegasus} for CNNDM~\cite{}\todo{cite}, the Rouge-2 score for the top-beam generations from beam search is only 21.48.
% However, if we find the best ones from the top 15 generations from beam search results that have the maximum Rouge-2 score, the upper-bound performance can be 27.74.
% Moreover, if we combine the results from four different decoding methods and then choose the best output for evaluation, then the performance is 33.75, which has a 57\% improvement over the top-beam results.
% Similarly, the T5-large model on CommonGen~\cite{lin2019commongen} can have a 93\% gain on CIDEr\todo{cite}; the Opus-MT model~\cite{}\todo{cite} can have a 79.7\% gain on BLEU on WMT18 (zh-en).
% These oracle performances suggest that it is of vital importance to conduct re-ranking for candidate outputs for further improving LMs' performance in NLG tasks.



To quantitatively understand how sub-optimal the default selections of decoding methods are, we present an empirical analysis in Fig.~\ref{fig:oracle_hists} (and Tab.~\ref{tab:main_oracle_gap} in Appendix).
Here we look at three typical NLG tasks: summarization (CNN/DM), machine translation (WMT18), and constrained text generation (CommonGen), with their popularly used base models: PEGASUS ~\cite{zhang2020pegasus}, Opus-MT~\cite{opus_mt}, and T5-large~\cite{t5}. 
We can see that the default selections (yellow bars in Fig.~\ref{fig:oracle_hists}; the top-beam generations) are much worse than the oracle selections from the top 15 candidate generations for each decoding method (blue bars). 

Moreover, if we combine the results from the four methods as a larger candidate pool, then the performance (green bars) of these NLG models can be much improved. 
For example, the Rouge-2 score of PEAGUS can be improved by 57\% and the BLEU score for Opus-MT can be improved by nearly 80\%, compared to their top-beam performance. 
Simply put, the default selections (i.e., the generations with the highest decoding scores) are much worse than the best selections from a relatively small candidate pool. 
Therefore, we argue that it is of significant importance to rerank generation candidates in order to enhance the performance of LMs in NLG tasks.
% These oracle performances highlight the importance of re-ranking candidate outputs in order to further improve the performance of LMs in NLG tasks.
% For example, using the PEAGUS model~\cite{zhang2020pegasus} on the CNNDM dataset~\cite{Hermann2015TeachingMT}, we find that the Rouge-2 score for the top beam search generation is only 21.48. However, by selecting the best output from the top 15 beam search results based on the maximum Rouge-2 score, the upper-bound performance can be increased to 27.74. 
% Further improvement can be achieved by combining the results from four different decoding methods and selecting the best output for evaluation, resulting in a performance of 33.75, a 57\% increase over the top beam search results. Similarly, the T5-large model on the CommonGen dataset~\cite{lin2019commongen} can achieve a 93\% gain in CIDEr score; the Opus-MT model~\cite{Tiedemann2020OPUSMTB} can achieve a 79.7\% gain in BLEU on the WMT18 (zh-en) translation task~\cite{Bojar2018FindingsOT}. 


% This gap between oracle selections and top-ranked has been seen as a consequence of the exposure bias caused by the teacher-forcing paradigm for most auto-regressive models. 
% Reranking the candidates after decoding is a straightforward yet effective way to mitigate this gap and there are several recent works exploring this direction.
% For example,
% SimCLS \cite{Liu2021SimCLSAS} uses a simple contrastive training objective to train a reranker.
% The reranker in SimCLS basically uses the same encoder to encode the source text and each candidate output, and then uses the cosine similarities for scoring each candidate individually.
% A more recent successful method is SummaReranker (SR)~\cite{Ravaut2022SummaRerankerAM}, which aims to use mixture-of-experts training to improve the reranker for multiple metrics at the same time.
% The encoding module for reranking in SR is based on a cross-encoder, meaning that it accepts the concatenation of a source and a candidate target in a single input sequence, and then outputs a score for the candidate.
% Such a cross-encoder design in SR makes great use of the attention layers in Transformer architecture~\cite{vaswani2017attentionia} and further enhances the ability to score a candidate with the context of source inputs.

Why do decoding algorithms often overlook generation candidates of better quality? The lower quality of default selections is often attributed to the exposure bias caused by the teacher-forcing paradigm in most auto-regressive models. 
Plus, the greediness of the search process and the randomness in sampling are also part of the reasons.
Re-ranking has been a simple yet effective post hoc approach to mitigate this gap. 
For instance, MLM-scoring~\cite{mlmscoring} uses an external LM such as BERT to estimate the quality of a candidate without any supervision.
SimCLS \cite{Liu2021SimCLSAS} trains a re-ranker using a simple contrastive training objective, which encodes the source text and each candidate output using the same encoder and scores each candidate based on the cosine similarity between the embeddings. 
Another successful approach is SummaReranker (SR)~\cite{Ravaut2022SummaRerankerAM}, which is trained to improve the re-ranker for multiple metrics simultaneously. 

% The encoding module in SR is based on a cross-encoder, which takes the concatenation of a source and a candidate target as a single input sequence and produces a score for the candidate. This cross-encoder design leverages the attention layers in the Transformer architecture~\cite{vaswani2017attentionia} and further enhances the ability to score candidates in the context of the source inputs.



% Most prior reranking methods, such as SimCLS and SummaReranker, focus on individually scoring each candidate output given an input.
% We argue such individual scoring methods are limited because they never directly learn to examine the differences between candidates. 
% In practice, the candidates for reranking are mostly similar to each other and the advantage of one over the other is very subtle, considering that the candidates for reranking are already ranked top by some decoding methods. 
% Thus, we believe a dedicated pairwise comparison method is of more importance, which can carefully examine the subtle differences between a pair of candidates at a time and then rerank all candidates.

Prior reranking approaches have primarily focused on individually scoring each candidate's output based on a given input. 
Note that the differences between the candidates are usually very subtle since they all are ranked highly by some decoding methods.
If we cannot compare two candidates side by side, it is hard to individually measure the quality of a candidate even for humans.
Therefore, such individual scoring methods can be very limited because their encoders have never seen a pair of candidates at the same time.
We argue that a dedicated \textit{pairwise} comparison method is necessary to identify subtle differences between two candidates, thus improving the reranking performance.

% To this end, we propose a novel reranking method named \textsc{PairReranker}.   
% The key idea of our method is to jointly encode a source input and a pair of candidates (i.e., three items) with a single encoder and then use a pairwise loss function for learning to compare.
% Our extensive experiments on three NLG tasks (i.e., summarization, translation, and constrained sentence generation) show that \textsc{PairReranker} outperforms the baseline methods by a consistent margin and it is also compatible with very large language models such as GPT-3~\cite{}.

To this end, we propose a novel reranking method, \textsc{PairReranker}, the key idea of which is to jointly encode a source input and a pair of candidates (i.e., three items) with a single encoder and then use a pairwise loss function for learning to compare. We compute the comparison matrix and utilize it for our proposed full comparison methods. We analyze the efficiency trade-offs of them and also propose the bubble run inference method to improve the efficiency and keep the performance as well. Our experiments also prove its extensibility for large language models like GPT-3.
% \todo{add sentence about using matrix to get final ranked list; talk about the efficiency issues; and its extensibility to GPT-3 style models.}

Extensive experiments conducted on three NLG tasks (i.e., summarization, translation, and constrained sentence generation) demonstrate that \textsc{PairReranker} outperforms the baseline methods by a consistent margin and is also compatible with very large language models such as GPT-3 (text-davinci-003).
\textsc{PairReranker} not only outperforms the previous SOTA method SummaReranker on the summarization task, but also shows great generalization performance in the other two NLG tasks, which are not evaluated previously. 
In addition, our \textsc{PairReranker} can be transferred to improve GPT-3 results by 26.53\% and 11.65\% for CommonGen and WMT18 (zh-en) respectively, even though our rerankers are not trained with any candidates decoded by GPT-3 models.  

\todo{List our contribution more clearly. --> 1) problem, 2) dataset, 3) methods, 4) results and open-source repo}

% To sum up, our contributions are as follows: 
% \begin{itemize}
%     \item We propose 
% \end{itemize}
% To sum up,  \textsc{PairReranker} is a novel reranking candidate in NLG tasks. Its use of a single encoder and pairwise loss function allows for improved performance and compatibility with larger language models. The strong results in multiple NLG tasks and the ability to transfer to GPT-3 further demonstrate the versatility and potential of \textsc{PairReranker} for use in a variety of NLG applications.







% \todo{summarize the performance here}

==> sections/4_evaluation_old.tex <==




\section{Evaluation}
\label{sec:eval_old}
% In this section,
% we first introduce the three tasks and 
%  their datasets used for evaluation.
% We then introduce the baseline models and the specific evaluation setups.
% We present the main results in 

\subsection{Tasks and data creation}

We evaluate reranking methods on the following public dataset: CNN/DM, CommonGen, and WMT18 (zh-en). The data statistics of these benchmarks are in Table~\ref{tab:dataset_stat} (in Appendix).



\paragraph{CNN/DM} \cite{Hermann2015TeachingMT} is a dataset constructed from CNN and DailyMail websites. It is first used for machine-reading and comprehension, and later \citet{Nallapati2016AbstractiveTS} use it for abstractive summarization. Evaluation metrics are Rouge-1, Rouge-2, and Rouge-L. 


\paragraph{CommonGen} \cite{lin2019commongen} is a dataset used for generative commonsense reasoning. It contains 79K commonsense descriptions where the language model is required to compose a realistically plausible sentence from given concepts. Evaluation metrics are BLEU and CIDEr. 

\paragraph{WMT2018} \cite{Bojar2018FindingsOT} is a well-known dataset for evaluate machine translation. Here we use the Chinese-English split for evaluation. Evaluation metrics are BLEU. 


\subsection{Base models}

For the summarization task on CNN/DailyMail dataset, we use the famous PEGASUS-large~\cite{zhang2020pegasus} and BART-large~\cite{lewis2019bart}, which have exhibited great ability for abstractive summarization. We use the public fine-tuned checkpoint from Hugging face.
For the generative commonsense reasoning task on CommonGen dataset, we use the T5-large \cite{t5}. It's one of the vanilla baselines reported in \citet{lin2019commongen}. 
For the Chinese-English translation task on WMT18 dataset, we use the public pre-trained opus-mt checkpoint~\cite{Tiedemann2020OPUSMTB}.




\subsection{Evaluation setups}
\label{sec:evaluation_setup}

In this section, we talk about the training and testing paradigm of our reranker, including how we construct the training, validation, and testing dataset for our reranker, how we generate candidates, and what our experiment focuses on.


To construct the training dataset for the reranker, we need to ensure the base model used to generate candidates on the training dataset should never have seen these candidates. Otherwise, the reranker will be trained on the candidates with higher quality compared to the candidates that it will be tested on, which we found will result in fairly bad performance. Therefore, following \citet{Ravaut2022SummaRerankerAM}, we first fine-tune the original non-finetuned pre-trained model on half of the training dataset, which gives us 2 half-finetuned base models that each of them has only seen their own half of the training dataset. Then we use them to generate candidates on their un-seen half of the training dataset using the decoding method talked about before. These generated candidates together form a whole training dataset with generated candidates that resemble the quality during the inference stage. 

During the inference stage, we directly adopt the public checkpoints that have been finetuned on the whole training dataset. We generate candidates on the validation and test datasets with this public checkpoint, which constitutes the validation and testing datasets on which our reranker runs inference.
We use two decoding methods, beam search, and diverse beam search, in the experiments, following the prior work of SummaReranker. 
We generate 15 candidates for each decoding method for both training and inference. 



\subsection{Main results}
\label{main results}

% First, we investigate the oracle reranking gap for each dataset with respect to each decoding method. For each decoding method, we generate 15 candidates.
 

\paragraph{Overall performance in summarization.}
% \todo{Simply introduce Table 3 and highlight our gain. maybe also talk bout the gain in R-2 and R-L , .}



Following the training and testing paradigm stated in section \ref{sec:evaluation_setup}, we briefly report the test results on the CNN/DM dataset in Tab.~\ref{tab:cnndm_results}. With fine-tuned PEGASUS-large as the base model. our \textit{Max Logits} method improves the candidates' quality by 6.35\% in Rouge-1, which is higher than our baseline SummaReranker. Besides, the performance gains in other metrics like Rouge-2 (9.62\%) and Rouge-L (6.25\%) are also obviously better. 


\paragraph{Can PairReranker generalize to other generation tasks?}
Yes. In order to test the task generalization ability of our method, we here report the test results on CommonGen and WMT2018 (zh-en) in Tab.~\ref{tab:commongen_results} and Tab.~\ref{tab:wmt2018_results}. From the data in the table, our method also improves the candidates' quality significantly after reranking. Our \textit{Max Logits} method obtain a 2.45\% performance gain in CIDEr on the CommonGen dataset and a 6.12\% performance gain in BLEU on the WMT2018 dataset. What's more, it's worth noting our \textit{bubble run} method achieves an even higher gain in CIDEr (2.91\%).


We also report the performance of SummaReranker on the two datasets. In contrast to the great performance on summarization, SummaReranker seems to fail to generalize well on other datasets. We also find that SummaReranker obtains a decreased gain on the CommonGen dataset (-1.23\% in CIDEr). The improvement on the translation dataset is not obvious (0.57\% in BLEU). We hypothesize that this is because of the average length of the candidates and the target text in these two datasets are all significantly smaller than the one in summarization (see in Tab.~\ref{tab:dataset_stat}). Therefore, the higher in-group similarity brought by the shorter length makes it harder for SummaReranker to capture their difference. On the contrary, our method with direct attention between a pair of candidates could easily tackle this problem. 








\paragraph{Can PairReranker generalize other large-scale models like GPT-3?}
Yes. 
\textcolor{blue}{After training on an expert dataset, our reranker could directly be applied to other models' outputs selection for the same task. To support this, we directly apply our three rerankers trained on the 3 main tasks respectively to the GPT-3 outputs with proper task-specific prompts.
} 
We report the performance gain in Tab.~\ref{tab:cnndm_results}, ~\ref{tab:commongen_results}, and~\ref{tab:wmt2018_results}. From the data reported in the table, we could see that the quality of the GPT-3 outputs is improved by a large margin compared to the average. Also, our performance gain is significantly larger than the baseline SummaReranker. For example, on the GPT-3 data points sampled from CNN/DM, our max logits method obtain a gain of 6.64\%, whereas SummaReranker only obtains a gain of 4.37\%. And on the CommonGen's, our method obtains a gain of 26.53\% and SummaReranker only obtains a gain of 18.79\%.

\input{tables/gpt3_results}

\begin{figure*}[t]
    % \vspace{-2em}
    % \centering
    % \hspace{-2.5em}
    \includegraphics[width=1.0\linewidth]{figures/tradeoff_merged.pdf}
    % \vspace{-3em}
    \caption{Efficiency trade-off with the number of pairwise comparisons \todo{consider move to the appendix, because this is about the traditional tasks}}
    \label{fig:tradeoff_merged}
\end{figure*}




\paragraph{Can I make trade-offs between performance and number of comparisons?}
% Figure~\ref{fig:tradeoff_merged} 
% \todo{Add paragraphs here.}

% \todo{R2: More detailed discussion about Max Logits, Max wins, Bubble. Including when to use which, cause that leads to the difference between them.}

Yes. Due to the high cost of full comparison methods, it's necessary for us to study the trade-off between the model performance and the number of comparisons.
% For full comparison methods, we first initialize matrix $M$ in Figure~\ref{fig:matrix} to be all zeroes, Then every time of the comparison, we fill a confidence cell that is zero before, then do the scoring and select the best one based on the current information in the matrix. For bubble run, we run multiple times of bubble run and select one that is chosen as the best one for the most times. Each bubble cost $N$ comparisons. The trade-off results are shown in Figure~\ref{fig:tradeoff_merged}.
From the results, we could see bubble run method could achieve high performance with little cost. However, as the number of comparisons increases, \textit{Max Logits} scoring methods will surpass the bubble run after a certain number of comparisons. 
\textcolor{blue}{We contend that the bubble run method already reports a pretty good performance with $N-1$ times of comparison. Therefore, most of the time, bubble run is a more efficient way to apply. If you want to pursue the marginal improvements brought by more comparison, you can also apply \textit{Max Logits} method with parallel computing.
}

% \paragraph{Does the input order affect the PairReranker?}
% % \todo{if any, talk about the order sensitivity in pairwise comparison; the order of the bubble sorting alg. }
% Due to the order of the input format, changing the position of candidate 1 and candidate 2 might also change the results (Sec. \ref{sec:architecture}). In practice, we record the frequency of these 2 results being consistent and found that by simply shuffling the order of candidate 1 and candidate 2, our reranker could be consistent with itself more than 90\% of the time. 


% \todo{Addition paragraph talking about the InstructGPT, as requested by R1}

\paragraph{}

	% - InstructGPT has reported that there is actually regression on the performance on some of the tasks, which is really bad. Long e.t. also did a a lot of efforts to fix that. However, our reranker could be used as an expert to recover the GPT-3's original great performance on these datasets after aligning through rearnking. And Our methods proves that it's quite easy to increase the performance on some of the dataset like cnndm, and commongen, with a much smaller NLU model like Roberta or Deberta. That's really impressive. 
	% - The Reward Model in InstructGPT is used for different ways from ours rerankers, though the training paradigm might resemble each other. 
	% - I could not give too many math explanations about this as bi-attention is indeed intuitively to be better than uni-attention




% \todo{
% Talk about the oracle gaps of the beam search and diverse beam search
% Create a 3-task version of Tab1 in SummaReranker. 
% }
% \todo{
% Talk about our results compared to the SimCLS, RefSum, SummaReranker.
% }
% \todo{The analysis and results on CommonGen and WMT2018; }


==> sections/__datasets.tex <==
\section{\mixdata \dataname{} Details}
\label{appendix:dataset}
As stated in ~\ref{ssec:dataset}, \dataname{} is constructed by collecting responses from 11 current popular LLMs, listed in ~\ref{tab:llm_results}. We here present the details of its construction.

We first deduplicate the dataset, then filter out the data points with too long or too short input and output. The length scope evaluated by the Llama tokenizer is constrained to be $[5,128]$. We shuffle the filtered data points and split them into train/val/test as 100k/5k/5k. Specifically for ShareGPT, we only take the first 2 items in the conversations as the input and output. That is, we only keep the first human input as the prompt and the following GPT outputs as the response. 

We use the top-p-sampling and set the temperature to 0.8. Except that, we keep all the other parameters as hugging face \texttt{Transformers} default values. For candidates from each model, we use 2 a6000 to do the inference for 72 hours to finish. Thus, the total a6000 time spent on generating is $2\times72\times11=1584(hours)=66(days)$.

% Following the success of famous ChatGPT, people start to build various open-source large language models based on the famous Llama~\cite{Touvron2023LLaMAOA}, Pythia\cite{Biderman2023PythiaAS} or others. However, how to evaluate these recently bloomed LLMs is one of the key issues in the NLP research community. To facilitate this process, LMsys has launched the ChatBot Arena project to collect human preferences on different models outputs in a pairwise way. It's the first well-known and effective LLM evaluation platform in the NLP research community. However, their evaluation results are currently not open-source and could be promote any further research on these models. 

% Besides, current LLM's research have mostly take the output from ChatGPT or GPT-4 as the de facto labels. We contend that the outputs from various other LLMs as well as their rank relationships for each single instruction and input are also sigificant. For example, we could use these rank relationships to train a reward model for RLHF or a reranker to select a better output from all these outputs from a various models.

% Therefore, we construct a dataset consists of various instructions and inputs as well as the outputs from today popular LLMs. This dataset is created by mixing 4 popular datasets used to finetune LLM to be instruction following.
% \begin{itemize}
%     \item GPT4all
%     \item Alapca data with gpt4 response
%     \item ShareGPT
%     \item Dolly15k
% \end{itemize}
% We first deduplicate the dataset, then filter out the data points with too long or too short input and output. The length scope evaluated by llama tokenizer is constrained to be $[5,128]$. We shuffle the filtered data points and split them into train/val/test as 100k/5k/5k. Specifically for ShareGPT, we only take the first 2 items in the converstations as the input and output. That is, we only keep the first human input as the prompt and the following gpt outputs as the response. The groud-truth outputs of these datasets are all created by ChatGPT, GPT-4 and Human.

% We generate the outputs with the following popular LLMs:
% \begin{itemize}
%     \item Stanford Alpaca
%     \item FastChat Vicuna
%     \item Dolly V2
%     \item StableLM
%     \item Open Assistant
%     \item Koala
%     \item Baize
%     \item Flan-T5
%     \item ChatGLM
%     \item MOSS
%     \item Moasic MPT
% \end{itemize}

% We use the top-p-sampling and set the temperature to be 0.8 and keep the other parameters as hugging face default values. For candidates from each model, we use 2 a6000 to do the inference for 72 hours to finish. 

% To evaluate the quality of these outputs, we use the traditional evalution metrics like BERTScore, Rouge and BLEU. In order to better understand the pair relationship between them, We also conduct pairwise comparison using ChatGPT on these outputs for the test split.




















==> sections/_alg.tex <==

\begin{algorithm}[t]
	\small 
    % \vspace{0.1em}
	\nonl \textbf{Input Data Clusters:}  {{$V_0, V_1, \dots, V_N$}} \\
% 	\vspace{0.1em}
	\nonl \textbf{Configuration Arguments}: $T, b, (\alpha, \beta, \gamma)$.  \\
% 	\vspace{0.1em}
	\nonl \textbf{Output}: A query stream $\{Q_1, Q_2, \dots, Q_T\}$
	%	\nonl {\scriptsize{/*~~*/}}
	
% 	\nonl{\textbf{Remarks}: $\Gamma_{n}(X)$ is a function to randomly sample $n$ unique elements from a set $X$.} \\ ~\\
	%	\comm{Add all tokens in to the token node set}
% 	\vspace{-1em}
	 
% 	\comm{Iterate each sampled distractor language $l_i$.} \\ 
	\ForEach{$t$ in $\operatorname{range}(1, T)$} { 
	   % $Q_t = [] $ ;
	   %\vspace{0.2em}
	    $b_u = \round{b * \alpha^{t-1}}$; $b_o = b -  b_u$ ; 
	    $b_o' = \round{b_o * \gamma} $ ; \\  
	   % \vspace{0.2em}
	    $c_t \sim P(c | c_{t-1}; \beta)$ \\
	   % \vspace{0.2em}
	    \comm{
	    The prob. of switching the major OOD data cluster is $1-\beta$, i.e.,
	    $P(c_t \neq  c_{t-1})=1-\beta$} \\
	   % \vspace{0.2em}
	    $V_{\neq c_t} = \bigcup_{\{k \in [1,N] | k \neq c_t\}} V_k$ \\ 
	   % \vspace{0.5em}
	    $Q_t {~\xleftarrow[]{}} \operatorname{sample}(V_0, b_u)$ \\ \comm{$V_0 \sim \mathcal{U}$; from upstream distribution} \\
		$Q_t \text{~+=~} \operatorname{sample}(V_{c_t}, b_o')$ \\ \comm{from the current major OOD data cluster} \\ 
		$Q_t \text{~+=~} \operatorname{sample}(V_{\neq c_t}, b_o-b_o')$ \\ \comm{from non-major data clusters}\\
% 		\comm{Add a distractor assertion as a candidate.}\\ 
% 		${C}$\text{.add}($M^{l_i}_j$)
        {$\operatorname{\textbf{assert}} ~|Q_t| = b$} 
        % \vspace{-1em}
	}
	\caption{\small{Sampling query streams with \textit{controllable non-stationarity} from multiple data clusters.}}\label{alg:cns}
\end{algorithm}



==> sections/_fig_heatmap.tex <==


\begin{figure}[t]
% \vspace{-1em}
	\centering
% 	\hspace{-0.5em}
	\includegraphics[width=1\linewidth]{figures/heatmaps.pdf}
	\caption{  The differences between refined models produced by different CMR methods in terms of their predictions for the same inputs at two time spans (10-20 and 30-40). The darker cells have large discrepancy.}
	\label{fig:heatmap}
\end{figure}



==> sections/_fig_methods.tex <==


\begin{figure*}[t]
% 	\centering
	\hspace{-0.5em}
	\includegraphics[width=1.03\linewidth]{figures/cmr_methods}
% 	\vspace{-1em}
	\caption{ The studied  methods for continual model refinement (Section~\ref{sec:methods}).  \vspace{-1em}}
	\label{fig:methods}
\end{figure*}
 

==> sections/_fig_metrics.tex <==


\begin{figure*}[t]
% 	\centering
	\hspace{-1em}
	\includegraphics[width=1.05\linewidth]{figures/cmr_metrics}
	\vspace{-1em}
	\caption{ The proposed five basic metrics for evaluating continual model refinement methods. \vspace{-1em}}
	\label{fig:metrics}
\end{figure*}
 

==> sections/_fig_stream.tex <==
 
\begin{figure*}[th!]
	\centering
% 	\hspace{-2em}
	\includegraphics[width=1\linewidth]{figures/submission_streams.pdf}
	\caption{\small The \textit{left} and \textit{middle} figures are two \textbf{query streams} of the QA task with different non-stationarity ($\beta=\{0.1, 0.5\}$) while sharing other arguments ($T$=50, $b$=64, $\alpha$=0.9, $\gamma$=0.8). 
	We use the blue color and `*' to denote the in-distribution data cluster (i.e., $V_0$), the percentage of which decay over time. 
	The distribution of incoming query examples dynamically shifts over time ---
	with larger $\beta$, adjacent episodes are more likely to share the same \textbf{major OOD clusters} which takes the $\gamma$ of the total OOD data.
	To encourage \textit{diversity}, the other $1-\gamma$ OOD examples are sampled from the remaining clusters.
	The \textit{right} figure is the \textbf{error stream} if we do not refine the upstream model (i.e., $f_t\equiv f_0$) and test it on the \textit{middle} query stream. } 
	\label{fig:submission_stream}
\end{figure*}

==> sections/_tab_main.tex <==

\begin{table*}[th!]
\centering
% \vspace{-1em}
% \hspace{-0.5em}
\scalebox{0.75}{
\begin{tabular}{r||c||cccc|c||cccc|c}
% \begin{tabular}{@{}lllllllll@{}}
\toprule
%  Question Answering $\rightarrow$ & - & \multicolumn{5}{c||}{\cellcolor{cyan!10}  } & \multicolumn{5}{c}{\cellcolor{blue!15} $()$ } \\ \midrule
  \textbf{Methods} $\downarrow$ \textbf{Metrics} $\rightarrow$ & \cellcolor{red!10} \AVG{EFR} & \cellcolor{blue!10} \AVG{UKR} & \cellcolor{blue!10} \AVG{OKR} & \cellcolor{blue!10} \AVG{CSR} & \cellcolor{blue!10} \AVG{KG} & \cellcolor{blue!10} \textbf{\AVG{OEC}} & \cellcolor{cyan!10} UKR\T & \cellcolor{cyan!10} OKR\T & \cellcolor{cyan!10} CSR\T & \cellcolor{cyan!10}KG\T & \cellcolor{cyan!10} \textbf{OEC\T} \\ \midrule 

 \rowcolor{gray!10}  Frozen Upstream ($f_t \equiv f_0$)  & 0.00  & 80.27 & 43.69 & 44.95 & 31.25 & 50.04 & 80.27 & 36.13 & 35.44 & 31.25 & 45.77 \\ \midrule
 {\color{gray}\ding{108}} \underline{Continual Fine-Tuning}   & 97.36 & 72.05 & 83.87 & 55.93 & 45.68 & 64.38 & 66.21 & 77.73 & 53.48 & 48.91 & 61.58 \\  \midrule 
{\color{brown}\ding{110}} \underline{Online L2Reg. }         & 97.18 & 73.47 & 85.37 & 57.27 & 47.12 & 65.81 & 71.09 & 83.59 & 54.50 & 51.17 & 65.09 \\
{\color[HTML]{7fc97f} \ding{115}} \underline{Online EWC}         & 97.49 & 73.38 & 86.09 & 56.17 & 47.34 & 65.75 & 68.55 & 85.74 & 53.67 & 53.28 & 65.31 \\ \midrule
{\color[HTML]{eb9634}\ding{58}} \underline{Exp. Replay (k=3)}    & 97.07 & 75.30 & 87.29 & 56.02 & 47.61 & 66.55 & 72.46 & 87.30 & 54.08 & 52.66 & 66.63 \\
Experience Replay (k=1)    & 96.72 & 78.91 & 89.38 & 57.80 & 47.17 & 68.31 & 78.13 & 86.52 & 55.33 & 52.73 & 68.18 \\ \midrule
% Dense Retrieval (k=1)      & 97.29 & 78.04 & 88.18 & 57.66 & 47.39 & 67.82 & 77.73 & 84.96 & 55.50 & 51.80 & 67.50 \\ \midrule
{\color[HTML]{c334eb} \ding{117}} \underline{MaxLoss (k=3,c=256)}      & 97.43 & 75.43 & 86.89 & 57.14 & 46.70 & 66.54 & 75.00 & 84.77 & 55.11 & 51.33 & 66.55 \\
MaxLoss (k=1,c=256)      & 96.54 & 78.16 & 89.86 & 57.78 & 46.63 & 68.11 & 77.54 & 89.26 & 55.47 & 50.94 & 68.30 \\
MaxLoss (k=1,c=512)       & 97.41 & 75.57 & 87.09 & 56.80 & 46.45 & 66.48 & 77.54 & 89.65 & 55.88 & 52.81 & 68.97 \\
MaxLoss (k=1,c=1024)   & 96.63 & 77.61 & 89.82 & 58.13 & 47.10 & 68.17 & 80.66 & 91.02 & 55.88 & 50.78 & 69.59 \\
 \midrule
% $\rhd$
{\color[HTML]{386cb0}$\righttriangle$} \underline{MIR (k=3,c=256)} & 97.08 & 75.92 & 87.13 & 56.91 & 47.22 & 66.79 & 75.78 & 87.50 & 54.53 & 51.80 & 67.40 \\
MIR (k=1,c=256)     & 96.59 & 77.84 & 89.77 & 58.35 & 47.28 & 68.31 & 79.49 & 90.43 & 55.91 & 51.25 & 69.27 \\
MIR (k=1,c=512)     & 96.96 & 77.86 & 89.41 & 58.13 & 46.40 & 67.95 & 79.69 & 89.45 & 55.50 & 50.08 & 68.68 \\
MIR (k=1,c=1024) & 96.71&	77.47&	87.83&	57.98&	46.87&	67.54&	78.13&	87.89&	55.73&	50.70&	68.11 \\ \midrule
{MIR(1,256)}+OnlineL2Reg          & 96.15&	79.10&	90.41&	59.80&	47.90&	69.30 & 79.49 & 90.04 & 57.45 & 52.66 & 69.91 \\
\midrule
 \rowcolor{gray!20}   Offline Refining ($f_0 \rightarrow f_T$)    & \textit{95.62} &	- & - & - &	- & - & \textit{83.78} & 	\textit{93.75} & \textit{93.81} &	\textit{56.17} &	\textit{81.88 }
%  0.837890625,0.9375,0.938125,0.56171875,0.81880859375
 \\
\bottomrule


\end{tabular}
}
\caption{\small Results (\%) in multiple metrics: \textbf{EFR}=Error-Fixing Rate; \textbf{UKR/OKR}=Upstream/Online Knowledge Retention; \textbf{CSR}=Cumulative Success Rate; \textbf{KG}=Knowledge Generalization. \textbf{OEC} is the average of the last four. Column names with bars are the average of all periods. The ones with `\T' are the scores at the final step.
The underlined methods are matched with the legends in Figure~\ref{fig:curves}. $k$ is the replay interval (the smaller the more frequent), and $c$ is the size of the candidate pool.  }
\label{tab:main}
\end{table*}


\begin{table}[htb]
\begin{center}
    \scalebox{0.75}{
    \begin{tabular}{c c c c c}
        \hline
         Decoding method & \# Candidates & R-1 & R-2 & R-L  \\
        \hline
        Top beam & 1 & 44.22 & 21.48 & 41.21\\
        \hline
         Beam Search & 15 & 51.06 & 27.74 & 48.05 \\
         Diverse Beam Search & 15 & 54.30 & 30.02 & 51.33\\
         Top-k sampling & 15 & 52.32 & 27.74 & 49.19 \\
         Top-p sampling & 15 & 53.51 & 28.83 & 50.40 \\
         \hdashline
         Adding all & 57.70 & 33.75 & 57.42 \\
        \hline
    \end{tabular}}
    \caption{\label{oracle_gap_cnndm} Oracle selection performance on CNN/Daily Mail using finetuned PEGASUS-large. Same as \citet{Ravaut2022SummaRerankerAM}}
\end{center}
\end{table}













==> sections/_tab_settings.tex <==

\begin{table}[t]
% \vspace{-1em}
\centering
% \hspace{-0.3em}
\scalebox{0.74}{
\begin{tabular}{r||ccccc}
\toprule 
 \textbf{Stream Dynamics}                              & \textbf{CFT}     & \textbf{EWC}   & \textbf{ER}      & \textbf{MxLs}   & \textbf{MIR}   \\ \toprule
 
% &  { $\\alpha$=0.9, $\\beta$=0.5, $\\gamma$=0.8} & 61.58  & 65.31  & 66.11  & 68.27  & 67.52   \\ \midrule
% &  $\\alpha$=0.9, $\\beta$=\textbf{0.1}, $\\gamma$=0.8 & 62.73  & 63.06  & 67.05  & 66.57  & 65.55  \\
% &  $\\alpha$=0.9, $\\beta$=\textbf{0.9}, $\\gamma$=0.8 & 64.58  & 65.32  & 67.50  & 67.23  & 67.22  \\  \midrule
% &  $\\alpha$=0.9, $\\beta$=0.5, $\\gamma$=\textbf{0.2} & 64.53  & 64.67  & 66.54  & 67.57  & 66.60   \\  
% &  $\\alpha$=0.9, $\\beta$=0.5, $\\gamma$=\textbf{0.5} & 63.86  & 64.62  & 66.02  & 64.75  & 65.85   \\\midrule
% &  $\\alpha$=\textbf{0.9}, $\\beta$=0.5, $\\gamma$=0.6 & 64.42  & 63.27  & 66.20  & 67.65  & 66.50  \\ 
 
%  $\alpha$=0.9, $\beta$=0.5, $\gamma$=0.8 & 61.6  & 65.3  & 66.1  & 68.3   & 67.5  \\ \midrule
%  $\alpha$=\textbf{0.1}, $\beta$=0.5, $\gamma$=0.8 & 64.5  & 64.7  & 66.5  & 67.6   & 66.6  \\ \midrule
%  $\alpha$=0.9, $\beta$=\textbf{0.1}, $\gamma$=0.8 & 62.7  & 63.1  & 67.1  & 66.6   & 65.6  \\
%  $\alpha$=0.9, $\beta$=\textbf{0.9}, $\gamma$=0.8 & 64.6  & 65.3  & 67.5  & 67.2   & 67.2  \\
%  \midrule
%  $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.2} & 63.9  & 64.6  & 66.0  & 64.8   & 65.8  \\
%  $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.5} & 64.4  & 63.3  & 66.2  & 67.6   & 66.5  \\
\rowcolor{gray!20} 
 $\alpha$=0.9, $\beta$=0.5, $\gamma$=0.8 & 15.81&	19.54&	20.86&	20.78&	21.63   \\ \midrule
%  $\alpha$=\textbf{0.1}, $\beta$=0.5, $\gamma$=0.8 & 17.29&	17.62&	21.62&	21.14&	20.12\\ \midrule
 $\alpha$=0.9, $\beta$=\textbf{0.1}, $\gamma$=0.8 & 23.40&	24.14&	26.32&	26.05&	26.04 \\
 $\alpha$=0.9, $\beta$=\textbf{0.9}, $\gamma$=0.8 & 18.61&	19.38&	20.78&	19.51&	20.60 \\
 \midrule
 $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.5} & 19.97&	20.10&	21.97&	23.01&	22.04 \\
 $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.2} & 17.37&	16.22&	19.15&	20.60&	19.45 \\
 \bottomrule


\end{tabular} 
}
\caption{\small The \textbf{\textit{gain}} of OEC\T over the \textit{Frozen Upstream} baseline for each method under different stream dynamics. \vspace{-0.5em}}
\label{tab:settings}
\end{table}


==> sections/staged.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}
\todo{this part can be removed at all or moved to the appendix.}
% \subsection{Background knowledge}


% \subsection{Formal description}
% \label{formaldescription}

Auto-regressive language models are trained by maximizing the log-likelihood for each token
$p\left ( y_t|y_{<t}, x\right )$, where $x$ is the given source sequence and $y$ is the ground-truth output. The overall training objective is
\begin{equation}
\theta^* = \mathop{\arg\max}_{\theta} \mathop{\mathbb{E}}_{x, y} {\left (\sum_{i}{\log{p(y_i|y_{<i},x})} \right )}.
\end{equation}

\noindent
During the inference time, the model is supposed to predict the next token based on the tokens generated by itself, which causes the mismatch between the training and inference stage. Each inference time, 
\begin{equation}
o_i = \mathop{\arg\max}_{o_i}p(o_i|o_{<i},x),
\end{equation}
where $o_i$ is the $i$-th output token generated by the model and $o_{<i}$ is the output tokens before $o_i$. This mismatch is referred to as exposure bias.

To bridge the gap brought by the exposure bias, reranking methods aim to select the candidate of higher quality generated by decoding methods. 
Let $\mathbb{D}=\{(x_1, y_1),...,(x_n,y_n)\}$ be the set of source-target text pairs for a specific language generation task. For the example $(x,y)$, let $C=\{c_{1}, ..., c_{m}\} \in \mathbb{C}$ be the corresponding generated candidates for source $x$. Thus the candidate of the highest quality with respect to metric $\mu \in \mathbb{M}$ is 
\begin{equation}
c^*=\mathop{\arg\max}_{c_i\sim C}\mu{(c_i, y)}.
\end{equation}



Without access to references,
a reranker $f_{\phi}$ should  give a higher score for $c^*$ than any other candidate $c_i$, where $\phi$ denotes the training parameters of the reranker $f$.
That is, \par

% Intuitively, the reranker is expected to
{\small{
\begin{equation}
\phi^* = \mathop{\arg\max}_{\phi} \mathop{\mathbb{E}}_{x,c_i\sim C}{\left( f_{\phi}(c^*,x)-\sum_i{f_{\phi}(c_i,x)} \right )}.%
\end{equation}
}
}


\noindent
An ideal reranker is thus expected to further select a better candidate than the default choices from decoding algorithms. It is especially important when we want to merge results from multiple different decoding algorithms and select the best ones.
Various training paradigms have been proposed to maximize this expectation. 
We present these baseline methods in Sec.~\ref{baseline methods}.

% \subsection{Challenges}
% \todo{why this is a hard problem.
% -- how we address these challenges.
% }

% % There are mainly two key challenges in training a reranker to evaluate the quality of the generated candidates. 
% % The first is the lack of references when we evaluate the candidate using $f_{\phi}(c_i,x)$. This requires the reranker to understand the source text and evaluate the candidate at the same time.

% The second challenge is the candidates are highly homogeneous which makes it difficult for the model to learn their difference. Different from traditional document retrieval where the document corpus is rich and heterogeneous, the search space of our problem only contains dozens of generated candidates from a normal language model. Therefore, how to train a reranker that could capture the subtle nuance among the candidates is what we will focus on. 
% \todo{Considering adding self bleu scores in this to demonstrate this point}

% \yuchen{will focus on the 2nd challenge and add more connections to our proposed methods}



==> tables/cmp_ranking_case.tex <==
\begin{table}[ht]
    \centering
    \scalebox{0.55}{
    \begin{tabular}{l l l}
        \hline
         \multicolumn{3}{c}{ CNN/Daily Mail}  \\
         \hline
        
\multicolumn{2}{l}{source(666)} &\makecell[l]{
(CNN)English actress Michelle Keegan has been named the sexiest woman in the world by British men's magazine FHM. \\
The 27-year-old actress is best known for her roles on the BBC series "Ordinary Lies" and the long-running British soap opera "Coronation Street." \\
Her "Coronation Street" character Tina McIntyre was the show's first character to act as a surrogate, according to IMDB. \\
Keegan is followed by reality television star and model Kendall Jenner, Oscar-winning actress Jennifer Lawrence,\\
Sports Illustrated swimsuit cover girl Kate Upton and British television host Caroline Flack, \\
who dated One Direction's Harry Styles for a few months. Sandra Bullock doesn't appear anywhere on FHM's list, \\
even though People magazine named her the "World's Most Beautiful Woman" a week ago. \\
The "FHM 100 Sexiest Women in the World" issue goes on sale Thursday, April 30.
} \\
\hline 

\multicolumn{2}{l}{target} &\makecell[l]{
British actress takes FHM's top spot in the list of 100 sexiest women in the world . \\
People's most beautiful woman is nowhere on the list .
} \\
\hline

\multirow{3}{8em}{Ours} & text & \makecell[l]{
"Ordinary Lies" actress Michelle Keegan is named sexiest woman in the world.<n>\\
Jennifer Lawrence, Kendall Jenner and Kate Upton also make FHM's list.<n>\\
Sandra Bullock doesn't appear on the list.
}\\
~ & scores & \makecell[l]{\text{Rouge-1: 44.07, Rouge-2: 17.54, Rouge-L: 40.68}} \\
~ & ranks & \makecell[l]{\text{Rouge-1: 1, Rouge-2: 1, Rouge-L: 1}} \\
\hline

\multirow{3}{8em}{SummaReranker} & text & \makecell[l]{
Michelle Keegan is best known for her roles on "Ordinary Lies" and "Coronation Street"<n>\\
Sandra Bullock doesn't appear on FHM's list.
}\\
~ & scores & \makecell[l]{\text{Rouge-1: 20.00, Rouge-2: 4.17, Rouge-L: 20.00}} \\
~ & ranks & \makecell[l]{\text{Rouge-1: 14, Rouge-2: 12, Rouge-L: 14}} \\
\hline

\multicolumn{2}{l}{source(156)} &\makecell[l]{
(CNN)Those poor fish must have been wondering what the heck was happening to them. \\
The Oregon Parks and Recreation Department has reported that a section of a fiberglass boat 20 or 30 feet long was \\
spotted off the state's coast this week and has been towed into harbor. \\
The debris is suspected to be from the earthquake and tsunami that hit Japan on March 11, 2011. \\
The boat fragment was found this week and towed to Newport, Oregon, where it is moored at a marina. \\
Inside were found -- more than four years and 4,000 miles later, if officials' suspicions are correct -- some specimens \\ 
of a variety of yellowtail jack fish normally found in Japanese waters. Biologists with the Oregon Coast Aquarium and \\
Oregon State University's Hatfield Marine Science Center inspected the debris while it was still at sea and determined \\
that the ecological threat posed by invasive species was small. The remnants of the boat will be dried out, \\
inspected further and taken to a landfill. But for the yellowtail jack fish, the journey is not over. \\
They'll be taken to the Oregon Coast Aquarium. 
} \\
\hline 

\multicolumn{2}{l}{target} &\makecell[l]{
Debris from boat to be dried, inspected and taken to landfill .\\
The debris contained fish normally found in Japanese waters .\\
The earthquake and tsunami hit Japan in March 2011 .
} \\
\hline

\multirow{3}{8em}{Ours} & text & \makecell[l]{
The debris is suspected to be from the 2011 earthquake and tsunami in Japan.<n>\\
The boat fragment was found this week and towed to Newport, Oregon.<n>\\
Inside were specimens of a variety of yellowtail jack fish normally found in Japanese waters.
}\\
~ & scores & \makecell[l]{\text{Rouge-1: 60.00, Rouge-2: 26.47, Rouge-L: 54.29}} \\
~ & ranks & \makecell[l]{\text{Rouge-1: 4, Rouge-2: 5, Rouge-L: 3}} \\
\hline

\multirow{3}{8em}{SummaReranker} & text & \makecell[l]{
A fiberglass boat fragment was found off the Oregon coast.<n>\\
It's suspected to be from the 2011 earthquake and tsunami in Japan.<n>\\
Inside were specimens of yellowtail jack fish.
}\\
~ & scores & \makecell[l]{\text{Rouge-1: 47.46, Rouge-2: 10.53, Rouge-L: 37.29}} \\
~ & ranks & \makecell[l]{\text{Rouge-1: 14, Rouge-2: 20, Rouge-L: 18}} \\
\hline

    \end{tabular}
} 

    \caption{Case studies.}
    \label{tab:cmp_ranking_case}
\end{table}

==> tables/gpt3_results.tex <==
\begin{table*}[!ht]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{@{}c || c c || c c || c c@{}}
            \toprule
             \multicolumn{1}{c}{\textbf{Datasets} $\rightarrow$}  &  \multicolumn{2}{c}{CNN/DailyMail} & \multicolumn{2}{c}{CommonGen} & \multicolumn{2}{c}{WMT18 (zh-en)} \\
             \toprule
             \textbf{Method} $\downarrow$ \textbf{Metric} $\rightarrow$ & R-2 & Gain$_{R2}$ & CIDEr & Gain$_{CIDEr}$ & BLEU & Gain$_{BLEU}$ \\
             \midrule
             \textbf{GPT-3} (text-davinci-003) & 15.51 & N/A & 11.12 & N/A & 23.61 & N/A \\ 
             \textbf{GPT-3}-oracle & 22.83 & 47.20\% & 19.26 & 73.20\% & 36.11 & 52.94\% \\
             GPT-3+MLM-Scoring & 15.09 & -2.71\% & 11.66 & 4.86\% & 23.98 & 1.57\% \\
             GPT-3+SummaReranker & 17.13 & 10.44\% & 13.21 & 18.79\% & 25.08 & 6.22\% \\
             \hdashline
             GPT-3+\textbf{PairRanker} (bubble) & 17.44 & 12.44\% & 13.85 & 24.55\% & 26.29 & 11.35\% \\
             GPT-3+\textbf{PairRanker} (max wins) & 17.46 & 12.57\% & 13.76 & 23.74\% & \textbf{26.36} & \textbf{11.65}\% \\
             GPT-3+\textbf{PairRanker} (max logits) & \textbf{17.54} & \textbf{13.09\%} & \textbf{14.07} & \textbf{26.53}\% & 26.19 & 10.93\% \\
            \bottomrule
        \end{tabular}
    }
    \caption{The performance gains on applying \texttt{PairReranker} to three conventional tasks, summarization, constrained text generation and translation.}
    \label{tab:gpt3_results}
\end{table*}


==> tables/main_oracle_gap.tex <==
\begin{table*}[h]
\begin{center}
    \scalebox{0.93}{
    \begin{tabular}{@{}c | c || c c c || c c || c@{}}
        \toprule
        \multicolumn{2}{c}{\textbf{Datasets} $\rightarrow$} & \multicolumn{3}{c}{CNN / DailyMail} & \multicolumn{2}{c}{CommonGen} & \multicolumn{1}{c}{WMT18(zh-en)} \\
        \toprule
         Decoding method $\downarrow$ & \# Candidates & R-1 & R-2 & R-L & BLEU & CIDEr & BLEU  \\
        \midrule
        Top beam & 1 & 44.22 & 21.48 & 41.21 & 14.62 & 15.48 & 19.20\\
        \midrule
         Beam search & 15$\rightarrow$ oracle & 51.06 & 27.74 & 48.05 & 23.62 & 24.56 & 25.84 \\
         Diverse beam search & 15$\rightarrow$ oracle& 54.30 & 30.02 & 51.33 & 23.58 & 23.61 & 26.08 \\
         Top-k sampling & 15$\rightarrow$ oracle & 52.32 & 27.74 & 49.19 & 21.66 & 21.44 & 19.60 \\
         Top-p sampling & 15$\rightarrow$ oracle & 53.51 & 28.83 & 50.40 & 22.78 & 22.82 & 20.84 \\
         \midrule
         All & 60$\rightarrow$ oracle& 57.70 & 33.75 & 57.42 & 30.04 & 29.89 & 34.51 \\
         Gain ($\frac{all-top}{top}\%$) & - & 30.5\% & 57.1\% & 39.3\% & 105.6\% & 93.0\% & 79.7\%\\
        \bottomrule
    \end{tabular}}
    \caption{\label{tab:main_oracle_gap} \small The empirical analysis of the oracle performance of decoding methods for three typical NLG tasks: summarization (CNNDM), constrained sentence generation (CommonGen), and machine translation (WMT18). Top beam is one of the most common methods of selecting output from beam searching results. However, the oracle selections in the top 15 candidates from four decoding methods are much better. If we use these four decoding methods jointly, the oracle performance gain is tremendous, as shown in the bottom row.}
\end{center}
\vspace{-2em}
\end{table*}
